GLEN: Generative Retrieval via Lexical Index Learning

Generative retrieval shed light on a new paradigm of document retrieval, aiming to directly generate the identifier of a relevant document for a query. While it takes advantage of bypassing the construction of auxiliary index structures, existing studies face two significant challenges: (i) the discrepancy between the knowledge of pre-trained language models and identifiers and (ii) the gap between training and inference that poses difficulty in learning to rank. To overcome these challenges, we propose a novel generative retrieval method, namely Generative retrieval via LExical iNdex learning (GLEN). For training, GLEN effectively exploits a dynamic lexical identifier using a two-phase index learning strategy, enabling it to learn meaningful lexical identifiers and relevance signals between queries and documents. For inference, GLEN utilizes collision-free inference, using identifier weights to rank documents without additional overhead. Experimental results prove that GLEN achieves state-of-the-art or competitive performance against existing generative retrieval methods on various benchmark datasets, e.g., NQ320k, MS MARCO, and BEIR. The code is available at https://github.com/skleee/GLEN.

==> Figures_tex/fig_pretrain.tex <==
\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=0.22\textwidth]{Figures/exp4_tmp.png} &
\includegraphics[width=0.22\textwidth]{Figures/exp4_tmp.png} \\
(a) NQ320k & (b) MS MARCO \\
\end{tabular}
\caption{Retrieval performance of GLEN depending on the different learning schemes.}
\label{fig:exp_pretrain}
\end{figure}

==> Tables/tab_collision_bm25.tex <==
\begin{table}[]\small
\centering
\setlength{\tabcolsep}{3pt} 
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{c|ccc|c}
\toprule
Datasets & \multicolumn{3}{c|}{NQ320k} & MS MARCO \\ \midrule
Metrics & R@1 & R@10 & MRR@100 & MRR@10 \\ \midrule
Random rerank & 67.7 & 82.4 & 74.5 & 16.6 \\
BM25 rerank & 68.9 & 86.0 & 75.3 & 19.2 \\ 
\bottomrule
\end{tabular}
\caption{Accuracy comparison of GLEN based on tie-breaking using the retrieval model in collision-free inference. We report the results using BM25~\cite{SIGIR/RobertsonW94/BM25}.}
\label{tab:exp_collision_bm25}
\end{table}

